Analysis of Measurements in a Microwave Oven with High Level of Non-Ionizing Radiation (NIR) Before and After Repair

Non-ionizing radiation is the subject of several applications, such as the microwave oven, which is very popular. Its use is characterized by direct user operation and reduced distances between users and the NIR source. Therefore, the level of human exposure in this scenario deserves attention as it is a potential cause of biological effects. In this sense, this paper presents the measurement of a microwave oven with a high level of NIR (above the limit defined by the standard) before and after two types of suggested repairs: the use of epoxy putty (Repair 1) and the replacement of the external surface of the oven (Repair 2). The definitions of measurement methodology, based on FDA and INMETRO standards, are presented and discussed. Finally, we describe an analysis of the efficiency of these repair methods aiming at the safety operation.

==> JCIS_RNI_Letter_forno_outlier/acronyms.tex <==
\begin{acronym}
  \acro{1G}{First Generation}
  \acro{2G}{Second Generation}
  \acro{3G}{Third Generation}
  \acro{4G}{Fourth Generation}
  \acro{5G}{Fifth Generation}
  \acro{5GRA}{Remote Areas applications}
  \acro{5GPHY}{5G Physical Layer}
  \acro{ADC}{analogic-to-digital converter}
  \acro{AGC}{automatic gain control}
  \acro{ASIP}{Application Specific Integrated Processors}
  \acro{AWGN}{additive white Gaussian noise}
  \acro{BDTM}{burst data transfer mode}
  \acro{BER}{bit error rate}
  \acro{BS}{base station}
  \acro{CDTM}{continuous data transfer mode}
  \acro{CFO}{Carrier Frequency Offset}
  \acro{CHF}{Characteristic Function}  
  \acro{CoMP} {Cooperative Multi-point}
  \acro{CP}{cyclic prefix}
  \acro{CR}{Cognitive Radio}
  \acro{CS}{cyclic suffix}
  \acro{CSI}{channel state information}
  \acro{CSMA}{carrier sense multiple access}
  \acro{DFT}{discrete Fourier transform}
  \acro{DPD}{digital pre-distortion}
  \acro{DZT}{discrete Zak transform}
  \acro{eMBB}{enhanced mobile broadband}
  \acro{EPC}{evolved packet core}
  \acro{FBMC}{Filter-bank multi-carrier}
  \acro{FDE}{frequency-domain equalizer}
  \acro{FDMA}{frequency division multiple access}
  \acro{FD-OQAM-GFDM}{frequency-domain OQAM-GFDM}
  \acro{FEC}{forward error control}
  \acro{FPGA}{Field Programmable Gate Array}
  \acro{FTN}{Faster than Nyquist}
  \acro{FT}{Fourier transform}
  \acro{FSC}{frequency-selective channel}
  \acro{GFDM}{Generalized Frequency Division Multiplexing}
  \acro{GS-GFDM}{guard-symbol GFDM}
  \acro{HPA}{high power amplifier}
  \acro{IBI}{inter-block interference}  
  \acro{ICI}{inter-carrier interference}
  \acro{IDFT}{Inverse Discrete Fourier Transform}
  \acro{IFI}{inter-frame interference}
  \acro{IMS}{IP multimedia subsystem}
  \acro{IoT}{Internet of Things}
  \acro{IP}{Internet Protocol}
  \acro{IQ}{in-phase and quadrature}
  \acro{ISI}{inter-symbol interference}
  \acro{IUI}{inter-user interference}
  \acro{KPI}{key performance indicator}
  \acro{LDPC}{low density check parity code}
  \acro{LLR}{log-likelihood ratio}
  \acro{LMMSE}{linear minimum mean square error}
  \acro{LTE}{Long-Term Evolution}
  \acro{LTE-A}{Long-Term Evolution - Advanced}
  \acro{M2M}{Machine-to-Machine}
  \acro{MA}{multiple access}
  \acro{MAC}{medium access control layer}
  \acro{MF}{Matched filter}
  \acro{MIMO}{multiple-input multiple-output}
  \acro{MMSE}{minimum mean square error}
  \acro{MRC}{maximum ratio combiner}
  \acro{MSE}{mean-squared error}
  \acro{mMTC}{massive machine type communication}
  \acro{MTC}{machine type communication}
  \acro{MU}{multi user}
  \acro{NEF}{noise enhancement factor}
  \acro{NFV}{network functions virtualization}
  \acro{OFDM}{Orthogonal Frequency Division Multiplexing}
  \acro{OOB}{out-of-band}
  \acro{OQAM}{Offset Quadrature Amplitude Modulation}
  \acro{PAPR}{peak to average power ratio}
  \acro{PHY}{physical layer}
  \acro{PRBS}{Pseudo Random Bit Sequence}
  \acro{PSD}{Power Spectrum Density}
  \acro{QAM}{quadrature amplitude modulation}
  \acro{QPSK}{quadrature phase shift keying}
  \acro{QoE}{Quality of Experience}
  \acro{QoS}{Quality of Service}
  \acro{RC}{raised-cosine}
  \acro{RF}{radio frequency}
  \acro{ROF}{roll-off factor}
  \acro{RRC}{root raised cosine}
  \acro{SC}{single carrier}
  \acro{SC-FDE}{Single Carrier Frequency Domain Equalization}
  \acro{SC-FDMA}{Single Carrier Frequency Domain Multiple Access}
  \acro{SCD}{Successive Cancellation Decoding}
  \acro{SDN}{software-defined network}
  \acro{SDR}{software-defined radio}
  \acro{SDW}{software-defined waveform}
  \acro{SEP}{symbol error probability}
  \acro{SER}{symbol error rate}
  \acro{SIC}{successive interference cancellation}
  \acro{SISO}{single-input single-output}
  \acro{SMS}{Short Message Service}
  \acro{SNR}{signal-to-noise ratio}
  \acro{ST}{space-time}
  \acro{STO}{Symbol Timing Offset}
  \acro{STC}{space time code}
  \acro{STFT}{short-time Fourier transform}
  \acro{TD-OQAM-GFDM}{time-domain OQAM-GFDM}
  \acro{TR-STC}{time-reversal space-time coding}
  \acro{TR-STC-GFDMA}{TR-STC Generalized Frequency Division Multiple Access}
  \acro{TVC}{time-variant channel}
  \acro{TVWS}{TV white space}
  \acro{UHF}{Ultra High Frequency}
  \acro{URLL}{ultra-reliable low latency}
  \acro{V2V}{vehicle-to-vehicle}
  \acro{VHF}{Very High Frequency}
  \acro{V-OFDM}{Vector OFDM}
  \acro{ZF}{zero-forcing}
  \acro{W-GFDM}{windowed GFDM}
  \acro{WHT}{Walsh-Hadamard Transform}
  \acro{WLAN}{wireless Local Area Network}
  \acro{WLE}{widely linear equalizer}
  \acro{WLP}{wide linear processing}
  \acro{WRAN}{Wireless Regional Area Network}
  \acro{WSN}{wireless sensor networks}
  \acro{TLS}{transport layer security}
  \acro{BRICS}{Brazil, Russia, India, and South Africa}
  \acro{LPWAN}{low-power wide-area network}
  \acro{UE}{user equipment}
  \acro{GPS}{Global Positioning System}
  \acro{RFID}{Radio-frequency identification}
  \acro{CAN1}{Controller Area Network 1}
  \acro{CAN2}{Controller Area Network 2}
  \acro{P2P}{Peer-to-peer}
  \acro{ICIC}{inter-cell interference coordination}
  \acro{ACK}{acknowledgment}
\end{acronym}


